Pailitao-MMSearch: Building Native E-Commerce Multimodal Search Foundation

The evolution of e-commerce has fundamentally transformed how users search for products, shifting from simple text-based keyword queries to complex multimodal interactions that seamlessly combine product images, natural language descriptions, and mixed-intent instructions. However, existing approaches face a critical dilemma: single-modal specialist models, deployed independently for text retrieval, visual search, and voice recognition, operate in isolation and cannot handle cross-modal queries, while general-purpose vision-language models lack the domain-specific knowledge necessary for fine-grained product understanding, user behavior modeling, and commercial intent reasoning. In this work, we present Pailitao-MMSearch, one native e-commerce multimodal search foundation model designed to bridge this gap. Our approach introduces three key innovations: (1)HybSID (Hybrid Semantic ID);(2)a two-stage continual pre-training strategy; and (3)a hybrid reasoning post-training pipeline. Built upon Qwen and deployed on Taobao's Pailitao multimodal search platform, Pailitao-MMSearch achieves substantial improvements in online A/B testing, including up to +13.61\% in Gross Merchandise Volume (GMV) and +8.21\% in transaction volume compared to traditional multi-modal search pipeline, demonstrating the effectiveness of our native e-commerce multimodal search large language models.

==> Sections/4-method.tex <==
\section{Method} \label{method}

We present Pailitao-MMSearch, a native e-commerce multimodal search foundation model that reformulates e-commerce multimodal search as \emph{autoregressive product generation}. As illustrated in Figure~\ref{fig:overview}, our approach consists of three main components: (1)~HybSID, a hybrid product tokenization scheme which unifies discrete semantic codes with a continuous multimodal embedding for unified product understanding and generation (\S\ref{sec:hybsid}); (2)~a two-stage continual pre-training pipeline for e-commerce domain knowledge injection and general capability preservation (\S\ref{sec:cpt}); and (3)~a hybrid reasoning post-training pipeline that adapts the model to diverse search intents and tasks (\S\ref{sec:posttraining}).

\begin{figure}[t]
    \centering
    \fbox{\parbox{0.92\textwidth}{\centering \vspace{2cm} \textit{[Overall Architecture of Pailitao-MMSearch: Base VLM $\rightarrow$ HybSID Tokenization $\rightarrow$ Two-Stage CPT $\rightarrow$ Post-Training $\rightarrow$ Deployment]} \vspace{2cm}}}
    \caption{Overall framework of Pailitao-MMSearch. The system builds upon a vision-language foundation model, introduces HybSID for product tokenization, applies two-stage continual pre-training for domain adaptation, and performs hybrid reasoning post-training for downstream search tasks.}
    \label{fig:overview}
\end{figure}

\subsection{Problem Formulation}

Let $\mathcal{P} = \{p_1, p_2, \ldots, p_N\}$ denote the product catalog containing $N$ products, where each product $p_i$ is associated with multimodal information including a product image $I_i$, a textual title $t_i$, and structured attributes $a_i$ (e.g., category, brand, material). A user $u$ is characterized by a historical interaction sequence $\mathcal{H}_u = (p_{u,1}, p_{u,2}, \ldots, p_{u,T})$ representing their chronologically ordered browsing, clicking, and purchasing behaviors. A multimodal search query $q = (I_q, t_q)$ consists of an optional query image $I_q$ and optional free-form text $t_q$, where at least one modality is present.

The multimodal search task is formulated as: given a user $u$ with history $\mathcal{H}_u$ and a multimodal query $q$, generate a ranked list of relevant products $\hat{\mathcal{P}} \subset \mathcal{P}$ that satisfy the user's search intent. Pailitao-MMSearch approaches this as an autoregressive generation problem: the model directly generates product identifiers (in the form of HybSID tokens) conditioned on the multimodal query and user context.

\subsection{HybSID: Hybrid Semantic Product Tokenization}
\label{sec:hybsid}

A core challenge in generative product retrieval is how to represent products as sequences of tokens that can be autoregressively generated by a language model. Existing approaches based on Semantic IDs (SIDs)~\cite{tiger,dsi} employ residual quantization to encode product representations as sequences of discrete codes. While this approach enables generative retrieval and provides semantic generalization through the shared codebook structure, the information bottleneck of discrete quantization inevitably sacrifices fine-grained product discrimination. Products that are semantically similar but commercially distinct---such as a genuine branded item and a visually similar generic alternative---may receive identical SID codes, leading to retrieval ambiguity.

To address this limitation, we propose \textbf{HybSID} (Hybrid Semantic ID), which augments discrete semantic codes with a continuous multimodal embedding, enabling the model to simultaneously leverage the generalization benefits of discrete tokenization and the discriminative power of continuous representations.

\subsubsection{Discrete Semantic Codes via Residual Quantization}

For each product $p_i$, we first extract a dense multimodal representation $\mathbf{v}_i \in \mathbb{R}^d$ using a pre-trained multimodal encoder that jointly encodes the product image, title, and attributes. We then apply Residual Quantization (RQ)~\cite{rqvae} with $K = 3$ hierarchical levels to map $\mathbf{v}_i$ into a sequence of discrete codes:

\begin{equation}
    s_i^{(k)} = \arg\min_{j \in [M]} \left\| \mathbf{r}_i^{(k-1)} - \mathbf{c}_j^{(k)} \right\|_2, \quad k = 1, 2, 3
\end{equation}
where $\mathbf{c}_j^{(k)} \in \mathcal{C}^{(k)}$ is the $j$-th codeword in the $k$-th level codebook $\mathcal{C}^{(k)} = \{\mathbf{c}_1^{(k)}, \ldots, \mathbf{c}_M^{(k)}\}$ with $M$ entries, and the residual at each level is:
\begin{equation}
    \mathbf{r}_i^{(0)} = \mathbf{v}_i, \quad \mathbf{r}_i^{(k)} = \mathbf{r}_i^{(k-1)} - \mathbf{c}_{s_i^{(k)}}^{(k)}, \quad k = 1, 2, 3
\end{equation}

The resulting discrete SID sequence $\mathbf{s}_i = (s_i^{(1)}, s_i^{(2)}, s_i^{(3)})$ forms a coarse-to-fine product identifier: the first code captures broad categorical semantics, subsequent codes progressively refine within-category distinctions. These codes are added to the LLM's vocabulary as special SID tokens.

\subsubsection{Continuous Multimodal Embedding}

To complement the discrete codes, each product retains a continuous multimodal embedding $\mathbf{e}_i^{\mathrm{mm}} \in \mathbb{R}^{d'}$ that captures fine-grained product information beyond the resolution of quantized codes. This embedding is derived from the product's multimodal features and preserves discriminative details such as subtle visual patterns, attribute-level distinctions, and style characteristics.

In the generation paradigm, we introduce a shared special token \token{emb\_token} that serves as a \emph{placeholder} for continuous embedding generation. Unlike discrete SID tokens that are position-fixed, \token{emb\_token} can appear at any position in the generated sequence, enabling flexible interleaved generation of text and product representations. This design supports diverse output formats including single-product retrieval, multi-product recommendation lists, and text-interleaved product descriptions.

\subsubsection{Unified Understanding and Generation}

The complete HybSID representation for product $p_i$ is defined as:
\begin{equation}
    \mathcal{S}_i = \left(s_i^{(1)},\; s_i^{(2)},\; s_i^{(3)},\; \mathbf{e}_i^{\mathrm{mm}}\right)
\end{equation}

HybSID operates in two complementary modes:

\textbf{Understanding mode.} When a product appears in the model's input context (e.g., as part of user history or a reference product in the query), its HybSID representation is converted to the LLM's embedding space. The discrete codes are mapped through the standard token embedding lookup, while the continuous embedding is projected via a learned \textbf{HybProjection} module:
\begin{equation}
    \mathbf{x}_i = \left[\mathrm{Emb}(s_i^{(1)});\; \mathrm{Emb}(s_i^{(2)});\; \mathrm{Emb}(s_i^{(3)});\; \mathbf{W}_{\mathrm{proj}} \cdot \mathbf{e}_i^{\mathrm{mm}} + \mathbf{b}_{\mathrm{proj}}\right]
    \label{eq:understanding}
\end{equation}
where $\mathrm{Emb}(\cdot)$ denotes the token embedding function, $[\cdot;\cdot]$ denotes concatenation along the sequence dimension, and $\mathbf{W}_{\mathrm{proj}} \in \mathbb{R}^{d_{\mathrm{model}} \times d'}$ is the projection matrix.

\textbf{Generation mode.} When the model generates a product as output, it autoregressively produces the three discrete SID tokens followed by \token{emb\_token}. Upon generating \token{emb\_token}, the corresponding hidden state $\mathbf{h}_{\mathrm{emb}}$ at that position is passed through a learned \textbf{HybDecoder} to reconstruct the continuous multimodal embedding:
\begin{equation}
    \hat{\mathbf{e}}_i^{\mathrm{mm}} = \mathrm{HybDecoder}(\mathbf{h}_{\mathrm{emb}})
    \label{eq:generation}
\end{equation}

The HybDecoder is a lightweight MLP that maps from the LLM's hidden dimension to the multimodal embedding space. The reconstructed embedding $\hat{\mathbf{e}}_i^{\mathrm{mm}}$ can then be used for fine-grained product retrieval via nearest-neighbor search in the embedding space, complementing the coarse retrieval provided by the discrete SID codes.

\begin{figure}[t]
    \centering
    \fbox{\parbox{0.92\textwidth}{\centering \vspace{2.5cm} \textit{[HybSID Illustration: Left: Product $\rightarrow$ RQ Encoder $\rightarrow$ $(s^{(1)}, s^{(2)}, s^{(3)})$ + $\mathbf{e}^{\mathrm{mm}}$. Middle: Understanding path with HybProjection. Right: Generation path with \token{emb\_token} and HybDecoder.]} \vspace{2.5cm}}}
    \caption{Architecture of HybSID. Each product is represented by three discrete SID tokens obtained through residual quantization and one continuous multimodal embedding. In understanding mode (left), both components are projected into the LLM's embedding space. In generation mode (right), the model autoregressively generates SID tokens and a special \token{emb\_token}, whose hidden state is decoded into the continuous embedding via HybDecoder.}
    \label{fig:hybsid}
\end{figure}

The training loss for HybSID generation combines discrete and continuous objectives:
\begin{equation}
    \mathcal{L}_{\mathrm{hyb}} = \mathcal{L}_{\mathrm{CE}}\!\left(\hat{s}^{(1:3)}, s^{(1:3)*}\right) + \lambda \cdot \mathcal{L}_{\mathrm{emb}}\!\left(\hat{\mathbf{e}}^{\mathrm{mm}}, \mathbf{e}^{\mathrm{mm}*}\right)
    \label{eq:hybsid_loss}
\end{equation}
where $\mathcal{L}_{\mathrm{CE}}$ is the standard cross-entropy loss over the discrete SID tokens, $\mathcal{L}_{\mathrm{emb}}$ is a cosine similarity loss for the continuous embedding reconstruction, $*$ denotes ground-truth targets, and $\lambda$ is a balancing coefficient.

\subsection{Two-Stage Continual Pre-Training}
\label{sec:cpt}

Adapting a general-purpose VLM to the e-commerce domain requires injecting substantial domain knowledge while avoiding catastrophic forgetting of the model's general language understanding and reasoning capabilities. We address this through a carefully designed two-stage continual pre-training (CPT) pipeline, as illustrated in Figure~\ref{fig:cpt}.

\begin{figure}[t]
    \centering
    \fbox{\parbox{0.92\textwidth}{\centering \vspace{2cm} \textit{[Two-Stage CPT Pipeline: Stage 1 (Product Knowledge Alignment + User Behavior Alignment + Background NL) $\rightarrow$ Stage 2 (OPD with Base LLM as Teacher)]} \vspace{2cm}}}
    \caption{Two-stage continual pre-training pipeline. Stage~1 injects e-commerce domain knowledge through product knowledge alignment and user behavior alignment tasks, with a background natural language objective. Stage~2 applies On-Policy Distillation (OPD) using the original base LLM as a teacher to recover general language capabilities.}
    \label{fig:cpt}
\end{figure}

\subsubsection{Stage 1: E-Commerce Domain Knowledge Injection}

The first stage focuses on aligning the model with e-commerce domain knowledge through two complementary training objectives, supplemented by a background natural language task:

\textbf{Product Knowledge Alignment ($\mathcal{L}_{\mathrm{prod}}$).} This objective trains the model to understand individual products at a fine-grained multimodal level. Given a product $p_i$ with its image $I_i$, title $t_i$, and attributes $a_i$, the model learns to:
\begin{itemize}
    \item Generate product titles and attribute descriptions from images, establishing visual-to-textual grounding;
    \item Predict product categories, brands, and material properties from multimodal inputs;
    \item Reconstruct product HybSID representations from textual and visual descriptions, learning the mapping from natural language product specifications to tokenized product identifiers;
    \item Perform cross-modal matching between product images and their textual descriptions.
\end{itemize}

These tasks are formulated as autoregressive sequence generation, where the model produces target tokens conditioned on multimodal product context. The product knowledge alignment loss is:
\begin{equation}
    \mathcal{L}_{\mathrm{prod}} = -\mathbb{E}_{p_i \sim \mathcal{P}} \left[\sum_{l=1}^{L} \log P_\theta\!\left(y_l \mid y_{<l}, \mathcal{X}(p_i)\right)\right]
\end{equation}
where $\mathcal{X}(p_i)$ represents the multimodal input context for product $p_i$, $y_{1:L}$ is the target sequence (which may include text tokens and HybSID tokens), and $\theta$ denotes model parameters.

\textbf{User Behavior Alignment ($\mathcal{L}_{\mathrm{user}}$).} This objective captures collaborative signals and sequential patterns from user interaction data. Given a user's historical interaction sequence $\mathcal{H}_u = (p_{u,1}, \ldots, p_{u,T})$, the model learns to:
\begin{itemize}
    \item Predict the next product a user is likely to interact with, given their behavioral history represented as a sequence of HybSID tokens;
    \item Understand product co-occurrence patterns (e.g., users who buy phone cases also buy screen protectors);
    \item Capture preference transitions across sessions and contexts.
\end{itemize}

The user behavior alignment loss follows a next-item prediction formulation:
\begin{equation}
    \mathcal{L}_{\mathrm{user}} = -\mathbb{E}_{u} \left[\sum_{t=1}^{T} \log P_\theta\!\left(\mathcal{S}_{p_{u,t}} \mid \mathcal{S}_{p_{u,1}}, \ldots, \mathcal{S}_{p_{u,t-1}}\right)\right]
\end{equation}
where $\mathcal{S}_{p_{u,t}}$ is the HybSID representation of product $p_{u,t}$.

\textbf{Background Natural Language Task ($\mathcal{L}_{\mathrm{nl}}$).} To mitigate catastrophic forgetting during Stage~1, we include a small proportion of general-domain conversational data sampled from a distribution similar to the base model's original training data. This serves as a regularizer that prevents the model from drifting too far from its general language capabilities.

The overall Stage~1 training objective is:
\begin{equation}
    \mathcal{L}_{\mathrm{stage1}} = \alpha \cdot \mathcal{L}_{\mathrm{prod}} + \beta \cdot \mathcal{L}_{\mathrm{user}} + \gamma \cdot \mathcal{L}_{\mathrm{nl}}
    \label{eq:stage1}
\end{equation}
where $\alpha$, $\beta$, $\gamma$ are task-balancing coefficients.

\subsubsection{Stage 2: Language Capability Preservation via OPD}

While the background NL task in Stage~1 partially mitigates forgetting, we observe that the model's general language capabilities (instruction following, reasoning, dialogue coherence) still degrade noticeably after extensive domain pre-training. Since the original pre-training corpus of the base VLM is proprietary and inaccessible, we cannot simply replay it.

We address this through \textbf{On-Policy Distillation (OPD)}, which uses the \emph{original base VLM} as a teacher to restore the domain-adapted model's language capabilities. Specifically, given a set of general-domain prompts $\mathcal{D}_{\mathrm{gen}}$, we generate response pairs from both the base model $\pi_{\mathrm{base}}$ and the Stage~1 model $\pi_{\mathrm{s1}}$, and train the Stage~1 model to match the base model's output distribution on these general-domain tasks while retaining its acquired e-commerce knowledge:

\begin{equation}
    \mathcal{L}_{\mathrm{stage2}} = \mathcal{L}_{\mathrm{task}} + \mu \cdot D_{\mathrm{KL}}\!\left(\pi_{\mathrm{base}}(\cdot | x) \;\|\; \pi_{\mathrm{s1}}(\cdot | x)\right), \quad x \sim \mathcal{D}_{\mathrm{gen}}
    \label{eq:stage2}
\end{equation}
where $\mathcal{L}_{\mathrm{task}}$ continues the domain-specific objectives from Stage~1, $D_{\mathrm{KL}}$ is the Kullback-Leibler divergence, and $\mu$ controls the distillation strength.

This two-stage design effectively decouples the objectives: Stage~1 aggressively acquires domain knowledge without being constrained by general capability preservation, while Stage~2 systematically recovers general capabilities through targeted distillation. The resulting \textbf{Stage~2 CPT Model} serves as the foundation for all downstream post-training.

\subsection{Post-Training Pipeline}
\label{sec:posttraining}

Building upon the CPT foundation, we design a multi-phase post-training pipeline that progressively enhances the model's capabilities for diverse e-commerce multimodal search tasks.

\begin{figure}[t]
    \centering
    \fbox{\parbox{0.92\textwidth}{\centering \vspace{2cm} \textit{[Post-Training Pipeline: SFT Data Construction $\rightarrow$ Hybrid Reasoning SFT $\rightarrow$ RL Enhancement $\rightarrow$ Multi-Expert OPD $\rightarrow$ Final Model]} \vspace{2cm}}}
    \caption{Post-training pipeline overview. The CPT model undergoes multi-task SFT with difficulty-aware hybrid reasoning, followed by RL enhancement on hard tasks, and finally multi-expert OPD to fuse diverse capabilities into the final model.}
    \label{fig:posttraining}
\end{figure}

\subsubsection{Multi-Task SFT Data Construction}
\label{sec:sft_data}

The key to effective post-training lies in constructing high-quality supervised fine-tuning (SFT) data that covers the diverse search intents encountered in production. We design a systematic data construction pipeline grounded in real user behavior:

\textbf{Step 1: Candidate sample mining.} We extract candidate Query-Doc pairs from user behavioral trajectories across the entire platform. For each predefined search task type (Table~\ref{tab:tasks}), we apply task-specific heuristic rules to identify interaction patterns that match the task semantics. For instance, a user who sequentially clicks on a cup and then purchases a matching cup sleeve triggers the ``complementary recommendation'' rule, producing a candidate training pair.

\textbf{Step 2: Instruction generation.} Using the candidate Query-Doc pairs as anchors, we generate task-specific natural language instructions that describe the user's search intent. These instructions are synthesized to be diverse in phrasing while maintaining semantic consistency with the underlying task type.

\textbf{Step 3: Difficulty stratification and quality control.} Candidate samples are stratified by difficulty level (easy, medium, hard) based on the semantic distance between query and target product, the complexity of the search intent, and the number of modalities involved. We apply quality filters to ensure balanced task distribution and appropriate difficulty calibration for the SFT stage.

\begin{table}[t]
\centering
\caption{Multimodal search task types supported by Pailitao-MMSearch. Each task type corresponds to a specific user intent pattern and is associated with dedicated SFT training data.}
\label{tab:tasks}
\small
\begin{tabular}{llp{6cm}}
\toprule
\textbf{Task Type} & \textbf{Modality} & \textbf{Description} \\
\midrule
Similar Product Search & Image (+Text) & Find products visually and functionally similar to a reference image \\
Edit \& Modify Search & Image + Text & Find products matching the reference image with specific modifications (e.g., color, material) \\
Outfit Matching & Image + Text & Recommend complementary fashion items for outfit composition \\
Accessory Pairing & Image (+Text) & Suggest accessories or complementary products for a main item \\
Style-Based Search & Image (+Text) & Retrieve products matching a specific visual style or aesthetic \\
Divergent Recommendation & Image & Discover related but diverse products for exploration \\
\bottomrule
\end{tabular}
\end{table}

\subsubsection{Hybrid Reasoning: Direct Generation and Chain-of-Thought}
\label{sec:hybrid_reasoning}

Different search scenarios demand different levels of reasoning complexity. A straightforward similar product search may require only direct pattern matching, while a compound intent query (e.g., ``find a formal version of this casual dress in navy blue for a wedding'') requires multi-step reasoning about style transformation, color specification, and occasion appropriateness.

We adopt a \textbf{hybrid reasoning} approach that assigns reasoning strategies based on task difficulty:

\textbf{Direct generation} is applied to easy and medium difficulty samples, where the model directly generates the target product's HybSID given the multimodal query. This mode prioritizes inference efficiency and is suitable for the majority of production traffic.

\textbf{Chain-of-thought (CoT) reasoning} is applied to hard difficulty samples. For these complex scenarios, we construct CoT annotations that decompose the search intent into explicit reasoning steps:
\begin{enumerate}
    \item Identify and describe key attributes of the reference product
    \item Parse the user's modification or search intent
    \item Reason about the target product's expected attributes
    \item Generate the target product's HybSID
\end{enumerate}

The hybrid reasoning SFT is trained with a unified objective where the model learns to produce either direct outputs or CoT-augmented outputs depending on the input's difficulty signal:
\begin{equation}
    \mathcal{L}_{\mathrm{sft}} = -\mathbb{E}_{(x,y) \sim \mathcal{D}_{\mathrm{sft}}} \left[\sum_{l=1}^{|y|} \log P_\theta\!\left(y_l \mid y_{<l}, x\right)\right]
\end{equation}
where $y$ is the target response (either direct HybSID or CoT + HybSID) and $x$ is the multimodal query context.

\subsubsection{Reinforcement Learning with Verifiable Rewards}
\label{sec:rl}

For the challenging reasoning tasks, we further enhance the model through reinforcement learning (RL) with \textbf{verifiable, product-grounded rewards}. Unlike conventional RLHF~\cite{instructgpt} that relies on human preference judgments, our reward signal is derived from objective, automatically verifiable metrics:

\begin{equation}
    R(y \mid x) = \alpha_r \cdot \underbrace{\mathbb{1}\!\left[\hat{\mathbf{s}} = \mathbf{s}^*\right]}_{\text{SID Accuracy}} + \beta_r \cdot \underbrace{\mathrm{CosSim}\!\left(\hat{\mathbf{e}}^{\mathrm{mm}},\; \mathbf{e}^{\mathrm{mm}*}\right)}_{\text{Embedding Similarity}}
    \label{eq:reward}
\end{equation}
where $\hat{\mathbf{s}}$ and $\mathbf{s}^*$ denote the generated and ground-truth SID sequences respectively, $\hat{\mathbf{e}}^{\mathrm{mm}}$ and $\mathbf{e}^{\mathrm{mm}*}$ are the generated and ground-truth continuous embeddings, and $\alpha_r$, $\beta_r$ are reward weights.

This reward design has two key advantages: (1)~it is fully automatic and does not require human annotation, enabling scalable RL training over large datasets; (2)~it captures both coarse-level correctness (through SID accuracy) and fine-grained quality (through embedding similarity), providing a richer training signal than binary accuracy alone.

We apply Group Relative Policy Optimization (GRPO)~\cite{grpo} as the RL algorithm, which samples a group of responses for each query and uses relative rewards within the group to compute policy gradients, avoiding the need for a separate reward model:

\begin{equation}
    \nabla_\theta J(\theta) = \mathbb{E}_{x \sim \mathcal{D}} \left[\frac{1}{G} \sum_{g=1}^{G} \hat{A}_g \cdot \nabla_\theta \log \pi_\theta(y_g \mid x)\right]
    \label{eq:grpo}
\end{equation}
where $G$ is the group size, $y_g$ is the $g$-th sampled response, and $\hat{A}_g$ is the group-normalized advantage computed from the verifiable reward $R(y_g \mid x)$.

The RL phase produces task-specific \textbf{expert models}---for example, an expert specialized in complex outfit matching or compound intent reasoning---that achieve strong performance on their respective hard task domains.

\subsubsection{Multi-Expert On-Policy Distillation}
\label{sec:multiexpert}

The final stage fuses the capabilities of multiple specialized models into a single unified model through \textbf{Multi-Expert OPD}. We identify three types of expert models:

\begin{enumerate}
    \item \textbf{RL Expert Models}: Multiple task-specific models from the RL phase, each excelling at a particular type of complex search reasoning;
    \item \textbf{Base VLM}: The original vision-language model, which provides strong general natural language understanding and instruction-following capabilities;
    \item \textbf{SFT Model}: The hybrid reasoning SFT model, which serves as the base student model for distillation.
\end{enumerate}

The multi-expert OPD objective trains the student model to selectively absorb capabilities from each expert:
\begin{equation}
    \mathcal{L}_{\mathrm{meopd}} = \mathcal{L}_{\mathrm{sft}} + \sum_{k=1}^{K} w_k \cdot D_{\mathrm{KL}}\!\left(\pi_k(\cdot | x) \;\|\; \pi_{\mathrm{student}}(\cdot | x)\right)
    \label{eq:meopd}
\end{equation}
where $\pi_k$ represents the $k$-th expert model's policy, $w_k$ is the distillation weight for expert $k$, and the SFT loss $\mathcal{L}_{\mathrm{sft}}$ ensures the student retains its task-solving capabilities.

The final model inherits the domain-specialized reasoning of the RL experts, the general language capabilities of the base VLM, and the multi-task versatility of the SFT model, producing a comprehensive e-commerce multimodal search foundation model ready for production deployment.

